Towards Autonomous Visual Navigation in Arable Fields

Autonomous navigation of a robot in agricultural fields is essential for every task from crop monitoring to weed management and fertilizer application. Many current approaches rely on accurate GPS, however, such technology is expensive and also prone to failure (e.g. through lack of coverage). As such, autonomous navigation through sensors that can interpret their environment (such as cameras) is important to achieve the goal of autonomy in agriculture. In this paper, we introduce a purely vision-based navigation scheme that is able to reliably guide the robot through row-crop fields without manual intervention. Independent of any global localization or mapping, this approach is able to accurately follow the crop-rows and switch between the rows, only using onboard cameras. With the help of a novel crop-row detection and a novel crop-row switching technique, our navigation scheme can be deployed in a wide range of fields with different canopy types in various growth stages with limited parameter tuning, creating a crop agnostic navigation approach. We have extensively evaluated our approach in three different fields under various illumination conditions using our agricultural robotic platform (BonnBot-I). For navigation, our approach is evaluated on five crop types and achieves an average navigation accuracy of 3.82cm relative to manual teleoperation.

==> contribs/simulation.tex <==
Conducting experiments in field is always time consuming and costly. 
Hence, a proper and reliable simulator which can mimic the real world situations is priceless. 

Setting up a realistic simulated environment with realistic robots driving about may be a time consuming and tedious endeavor, while it pays back at the end. ?? !!!

Here, we introduce our simulation developed under Robotic Operating System (ROS), containing a one-to-one scaled simulation of BonnBot-I and a specific field simulator.

The robot model is containing all sensors an actuators which provided the capability to flawlessly test our algorithm without taking the real robot to the field. 
The figure \figref{fig:rviz_sim} depicts a full consultation of BonnBot-I in Rviz visualizer.
\begin{figure}[h]
	\centering
	\includegraphics[width=0.8\linewidth]{figures/rviz_tf}
	\caption{BonnBot-I Simulation. The overall structure of BonnBot-I including all sensors and actuators is depicted here. The robot description contains accurate TF-Tree and fully accessible sensory data.}
	\label{fig:rviz_sim}
\end{figure}

Offered simulation package is build upon the Saga \cite{grimstad2018software} provided simulation description of Thorvald platform, which then is being modified to meet our requirements. 
Primarily, we matched the dimension of the original description and then added all sensors weeding actuators according to our real robot.
Furthermore, WE developed a simulation package which is capable of generating a variety of field with different plants in size and shapes, the \figref{fig:frams} depicts some example generated fields. 
This packages is being used to develop our navigation strategies, too. 
